Style-A-Video: Agile Diffusion for Arbitrary Text-based Video Style Transfer

Large-scale text-to-video diffusion models have demonstrated an exceptional ability to synthesize diverse videos. However, due to the lack of extensive text-to-video datasets and the necessary computational resources for training, directly applying these models for video stylization remains difficult. Also, given that the noise addition process on the input content is random and destructive, fulfilling the style transfer task's content preservation criteria is challenging. This paper proposes a zero-shot video stylization method named Style-A-Video, which utilizes a generative pre-trained transformer with an image latent diffusion model to achieve a concise text-controlled video stylization. We improve the guidance condition in the denoising process, establishing a balance between artistic expression and structure preservation. Furthermore, to decrease inter-frame flicker and avoid the formation of additional artifacts, we employ a sampling optimization and a temporal consistency module. Extensive experiments show that we can attain superior content preservation and stylistic performance while incurring less consumption than previous solutions. Code will be available at https://github.com/haha-lisa/Style-A-Video.

==> Figures/moreresult2.tex <==
\begin{figure*}[thbp]
    \centering
    \includegraphics[width=\linewidth]{Images/more_result2_1.png}
    % \vspace{-0.2cm} 
    \caption{\textbf{More video style transfer results by Style-A-Video.} Our approach supports simple arbitrary style descriptions, without the necessity to describe the visual content in detail as \cite{tuneavideo,fatezero} require.
    }
    % \vspace{-0.4cm} 
    \label{fig:moreresult2}
\end{figure*}

==> Sections/5_failurecases.tex <==
\section{DISCUSSION}
% text2live
Our method has several limitations and is shown in Fig.~\textcolor{contentchange}{?}  shows these limitations. The first is the inability to accurately generate styles that are consistent with certain text hints. The possible reason for this is that the generative model does not have a strong prior for these contexts, limited by the distribution and amount of training data. The second failure is that the appearance of the subject changes due to the context of the cue, and there is an entanglement between the level style and the content. XXXX, for example, generates additional content related to the text.

Nevertheless, in many cases, the desired style editing can be achieved by adjusting the text. An example is XXXX.

==> Sections/6_sup.tex <==
\appendix

\input{Figures/unet}

\section{More Details of Implementation}

\subsection{U-Net Architecture}
The MGAD model adopts the U-Net~\cite{UNet} architecture shared across diffusion steps to generate $512 \times 512$ images. 
The architecture consists of seven downsampling and seven upsampling layers, as represented in Figure~\ref{fig:unet}. 
The model follows an encoder-decoder framework in conjunction with a time-step embedding module. 
For the encoder, the $4 \times 4$ feature map is generated from the $512 \times 512$ input image via one input convolution and seven residual blocks. 
One residual block comprises four convolutional blocks, including group normalization~\cite{wu2018group} and SiLU activation function~\cite{ramachandran2017searching}. At the $32 \times 32$, $16 \times 16$ and $8 \times 8$ resolutions, self-attention blocks are added to these residual blocks. 
Then, the encoder's $4 \times 4$ output is fed to a self-attention block before the decoder. 
For the decoder, the output whose resolution is the same as the input is produced through seven residual blocks and one output convolution with skip connections from the features in the encoder. 
For the time embedding module, the diffusion step $t$ is embedded into each residual block after the cosine wave encoding as proposed in \cite{vaswani2017attention}. 
Overall, the model receives ${x}_{t}$ and $t$ as inputs and outputs ${\epsilon}_{\theta}\left({x}_{t}, t\right)$.


\subsection{Implementation details}
We use the $512 \times 512$ unconditional ImageNet diffusion model, which is fine-tuned for $8,100$ steps from the OpenAI trained $512 \times 512$ class-conditional ImageNet diffusion model. 
It was fine-tuned into an unconditional model to enable better guidance by CLIP~\cite{openai}. 
Since the CLIP model receives the images with a resolution of $224 \times 224$, all images would be resized before feeding to the CLIP model. 
Besides, we use $L_{tv}$~\cite{LeonidIRudin1992NonlinearTV} to control the smoothness of the final output.
%and $L_{range}$ to control how far out of range RGB values are allowed to be. +\lambda_{range} L_{range} 
The total loss function of our model is formulated as:
\begin{equation}
L_{total}=\lambda_{MGS} L_{CLIP}+\lambda_{tv} L_{tv}.
\end{equation}
For hyperparameters, we usually set $\lambda_{MGS}$ and $\lambda_{tv}$ as $5,000$ and $300$, respectively.


\subsection{Training dataset}
The first diffusion model we used is an unconditional model fine-tuned from OpenAI's class-conditional ImageNet diffusion model~\cite{Guided-Diffusion} with $512 \times 512$ resolution. The secondary diffusion model~\cite{model} was pre-trained on the YFCC100m~\cite{yfcc100} dataset. We have also tried to train the secondary diffusion model on the WikiArt dataset. However, the generated results are over similar in style, influenced by the content, type, volume, and distribution ratio of the WikiArt dataset. As a result, it does not match well with the multimodal guidance prompts content. Our goal is to generate artistic images with high visual quality and improve the semantic relevance of the generated results to prompts. Therefore, the diffusion model trained on the YFCC100m~\cite{yfcc100} is used to maintain semantic consistency with the rich and variable artistic content of prompts.

% For the diffusion model, we used an unconditional model of resolution $512 \times 512$ fine-tuned from OpenAI's class-conditional ImageNet diffusion model~\cite{Guided-Diffusion}. Additionally, we use a secondary diffusion model~\cite{model} pre-trained on Yahoo Flickr Creative Commons 100 Million (YFCC100m)~\cite{yfcc100} dataset for better performance. 



% ###################################################################
\section{Additional Results}

\input{Figures/sup-baseline}
\input{Figures/steps_ddim}



In this section, we provide additional results of the MGAD. Firstly, we compare our results with two more baselines. Then, we show the results generated for different time steps. Besides, we compare the results of DDPM and DDIM in our framework. Lastly, we analyze the generation of MGAD model in open domain.

\subsection{More comparison results}
We compare the proposed MGAD with two additional baselines: 1) ``retrieve-restylization'', i.e., utilizing the text-retrieved image as the style image and then using the existing style transfer approach; 2) ``generation-restylization'', i.e., applying the image generated by the text-to-image generation model as the style image and performing style transfer as well. 
Regarding the ``retrieve-restylization'' pipeline, we selected the image with the maximum CLIP score as a style image by using the pre-trained text-to-image retrieval model~\footnote{\url{https://github.com/rom1504/clip-retrieval}}. 
Regarding the ``generation-restylization'' pipeline, we used the image created via VQGAN+CLIP~\footnote{\url{https://github.com/nerdyrodent/VQGAN-CLIP}} as a style image. Furthermore, we chose the arbitrary style transfer model AdaAttN~\cite{liu2021adaattn} as the style transfer method.

In Figure~\ref{fig:sup-baseline}, we can observe that the visual quality of these two-step baselines is highly dependent on  the retrieval and generation models. 
The final results will be substantially influenced if the qualities of the retrieved or produced style images are not high (e.g., the 4$^{th}$-7$^{th}$ rows in Figure~\ref{fig:sup-baseline}). 


We can observe that the outline and color of ``retrieve-restylization'' results (e.g., the 5$^{th}$ row in Figure~\ref{fig:sup-baseline}) are blurred. The transitions between different objects of the results obtained by ``generation-restylization'' are not natural enough (e.g., the 7$^{th}$ row in Figure~\ref{fig:sup-baseline}). A major difference from the stylized approach is that our results are similar to the image prompts to a certain extent but not completely bound to the structures of the image prompts (e.g., the 5$^{th}$ and 7$^{th}$ rows in Figure~\ref{fig:sup-baseline}). Thus, the paintings generated by our model clearly resemble real artworks in excess of the style transfer results (e.g., the 3$^{rd}$ row in Figure~\ref{fig:sup-baseline}).
In general, the MGAD model is more flexible and accessible for the synthesis of digital artworks.
%In general, the MGAD model is more flexible and accessible for artistic processing and creation, which is more conducive to the generation of digital artworks.

\subsection{The Impact of Time Steps}
To ensure the quality of the results and maintain the parameters' consistency, the experiments in this work used diffusion steps and time steps both set to 2000. Time steps determine the generation time. As the DDPM results are shown in the first and third rows of the Figure~\ref{fig:steps_ddim}, we found that when the diffusion steps were set to 2000 steps and the time steps were set to 500 steps, we could obtain good results. When the time steps were set to 1000 steps, the results were very close to those of 2000 steps.

\subsection{Comparison to DDIM}
We utilize Denoising Diffusion Probabilistic Models (DDPM) in our approach. A fast sampling algorithm for DDPM proposed by Song et al.~\cite{DDIM} is named Denoising Diffusion Implicit Models (DDIM). Nichol et al.~\cite{IDDPM} demonstrated that DDIM provides superior samples than DDPM with fewer steps, but inferior samples with 50 or more steps. Figure~\ref{fig:steps_ddim} shows the comparison of the experimental results using DDPM and DDIM in our framework. DDIM generates better results than DDPM when there are fewer steps. However, as the time steps increase, DDPM produces better results than DDIM.

\input{Figures/opendomain}
\subsection{Open-domain results}
We tried to use prefixed text prompts (e.g., "A photo of" + artistic comments) or non-artistic text prompts (e.g., "A photo of a landscape") as guidance~\ref{fig:opendomain}; however, the generated visual results are somewhat out of realistic domain whatever photo or painting is used as image prompts. Similar observations could be made from recent CLIP-based open domain image generation approaches such as BigSleep~\cite{bigsleep} and VQGAN+CLIP~\cite{Vqgan-clip-paper}. Though these methods focus on generating images in the open domain, most of their visual results are in the artistic domain. Based on the results of our experiments, CLIP is able to interpret artistic style in prompts with great understanding. The learned higher-level semantic concepts in CLIP are consistent with our motivation to generate digital artworks. Considering the significance and difficulty of creating digital artwork, our present work primarily focuses on this task. In the future, we will concentrate more on involving art stroke or model-based techniques.

% ###################################################################
\input{Figures/badcases}
\section{Bad Cases}
In this section, we show several failure cases of our model. 
Since our model is guided by both image and text prompts, failures could occur when the guidance of these prompts is overly inconsistent.
In the example of the first line of Figure~\ref{fig:badcases}a, we can observe that the text prompt conditions we entered are ``Picasso'', ``cityscape'' and ``cubism'', but the content of the image is ``Monet's painting of the Seine''.
The contents of the two types of prompts are pretty inconsistent, causing the result to fail. 
The same problem exists in the second line of the example. 
The text prompt ``mountains'' and the image prompt ``cityscape'' are not integrated. 
In this case, dropping a module will result in a complete outcome. 
We kept the text prompts and discarded the image prompts, and the results are shown in Figure~\ref{fig:badcases}b.







% ###################################################################
\section{More Digital Art Generation Results}


\input{Figures/sup-diversity}
\input{Figures/sup-diversity2}


In Figures~\ref{fig:sup-diversity},~\ref{fig:sup-diversity2},~\ref{fig:moreresults_page1} and~\ref{fig:moreresults_page2}, we show more digital art generation results of our model. 
These results demonstrate the performance of our model in terms of diversity and quality.



\input{Figures/moreresults_page1}
\input{Figures/moreresults_page2}






% ###################################################################
\section{Societal Impact}
With the advancement and widespread use of the Internet and mobile devices, digital artwork is receiving growing attention. We explored the competence of machines to create high-quality artworks with multimodal guidance and ultimately achieved fantastic results. However, the pre-trained models that we utilize are the outcomes of training on vast online text and image datasets, which contain inherent social biases. Furthermore, since our approach utilizes images and texts to control the generation of digital artworks, there may be negative social implications when users input malicious images and texts.

\section{Data License}
The pre-trained models used in our work are the YYFC1 model~\cite{crowsonkb}, $512 \times 512$ unconditional ImageNet diffusion model and ViT-B/32~\cite{openai}. According to the license of the above models~\footnote{\url{https://github.com/crowsonkb/v-diffusion-pytorch/blob/master/LICENSE}}$^,$\footnote{\url{https://the-eye.eu/public/AI/models/512x512_diffusion_unconditional_ImageNet/README.txt}}$^,$\footnote{\url{https://github.com/openai/CLIP/blob/main/LICENSE}}, we can use, copy, modify, merge, publish and distribute them for education purposes and academic research. 

% https://github.com/openai/CLIP/blob/main/LICENSE
% https://github.com/crowsonkb/v-diffusion-pytorch/blob/master/LICENSE
% https://the-eye.eu/public/AI/models/512x512_diffusion_unconditional_ImageNet/README.txt

\endinput

==> macros.tex <==
\usepackage{ifthen}
\usepackage{xcolor}

\definecolor{WeimingColor}{rgb}{0,0,0.8}
 
\definecolor{FanColor}{rgb}{0.8,0,0.8}
 

\newcommand{\weiming}[1]{{\color{WeimingColor} [Weiming: #1]}}
 
 
\newcommand{\fan}[1]{{\color{FanColor}[Fan: #1]}}
 

\newcommand{\warning}[1]{{\it\color{red} #1}}
\newcommand{\toremove}[1]{{\it\color{red} (To remove) #1}}
\newcommand{\note}[1]{{\it\color{blue} #1}}
\newcommand{\nothing}[1]{}

\ifthenelse{\equal{\final}{1}}
{
\renewcommand{\weiming}[1]{}
\renewcommand{\fan}[1]{}
 
 

\renewcommand{\warning}[1]{}
\renewcommand{\toremove}[1]{}
\renewcommand{\note}[1]{}
\renewcommand{\nothing}[1]{}
}{}

\hyphenpenalty=1000 % magic number to reduce ugly line breaks

\newcommand{\inputsection}[1]{\input{Sections/#1}}
\newcommand{\inputfigure}[1]{\input{Figures/#1}}
\newcommand{\inputtable}[1]{\input{Tables/#1}}

